Systematic Review of Lightweight Cryptographic Algorithms

The emergence of small computing devices and the integration of processing units into everyday objects has made lightweight cryptography an essential part of the security landscape. Conventional cryptographic algorithms such as AES, RSA, and DES are unsuitable for resource-constrained devices due to limited processing power, memory, and battery. This paper provides a systematic review of lightweight cryptographic algorithms and the appropriateness of different algorithms in different areas such as IoT, RFID, and wireless sensor networks. Using tabular analysis and graphical interpretation, we compare these algorithms in terms of performance, security, energy consumption, and implementation costs. An overview of the evolution of lightweight cryptography based on those design trade-offs is also provided.

==> Tables/01.Cipher_Summary_Tables/12_Summary_LWHF.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.5}
\scriptsize
\caption{Comparative Analysis of LHC Ciphers.}
\label{tab:CompAna_LWHF}
\begin{tabular}{l c l l}
\toprule
\textbf{Year} & \textbf{Resistant Against Attacks} & \textbf{Proven Vulnerabilities}
\\
\midrule
DM-PRESENT \cite{bogdanov2008hash} & 2008 & & Distinguisher (18-r); Second preimage (12-r)~\cite{koyama2013multi}
\\ 
\hline
QUARK \cite{aumasson2010quark} & 2010 & Collision; Preimage; Cube; Differential & Conditional differential~\cite{yang2018symbolic}; Side channel
\\ 
\hline
Lesamnta-LW \cite{hirose2010lightweight} & 2010 & Collision; Preimage; Second-preimage & Key-recovery (20-r); integral (18/19/25-r)~\cite{shiba2022integral}
\\ 
\hline
PHOTON \cite{guo2011photon} & 2011 & Related-key; Collision; Preimage & Differential fault analysis~\cite{li2018security}
\\ 
\hline
SPONGENT \cite{bogdanov2011spongent} & 2011 & Differential; Linear; Preimage; Collision
\\ 
\hline
LHash \cite{wu2013lhash} & 2013 & Differential; Impossible differential; Preimage; Collision &
\\
\hline
Blake 2 \cite{aumasson2013blake2} & 2013 & Second preimage; Side-channel; Length-extension & Key recovery rotational; Distinguisher~\cite{guo2014analysis}
\\ 
\hline
Neeva-Hash \cite{bussi2016neeva} & 2016 & Differential; Near-collision; Preimage & 
\\ 
\hline
Hash-One \cite{megha2016hash} & 2016 & Differential; Algebraic; Preimage; Collision
\\ 
\hline
HeW \cite{kumar2017hew} & 2017 & Differential; Linear; Slide; Rotational distinguisher
\\ 
\hline
L-CAHASH \cite{hanin2017cahash} & 2017 & Preimage; Second preimage &
\\ 
\hline
LNHASH \cite{9066107} & 2019 & Differential; Rebound; Algebraic; Rotational &
\\ 
\hline
LNMNT \cite{nabeel2021lnmnt} & 2021 & Collision; \ac{MITM} & \\
\bottomrule
\end{tabular} 
\end{table}

==> Tables/02.Hardware_Implementation_Tables/09_HW_Metrics_LWHF.tex <==
\begin{table} [H]
\scriptsize
\caption{Hardware implementation of Lightweight Hash Functions (LWHF).}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}l l l c c c c c c c}
\toprule
   & \multicolumn{2}{l}{\textbf{Hash Function}} &
  \textbf{Year} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Hash Size}\\ \textbf{(bits)}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Power} \\ \textbf{consumption}\\ \textbf{($\mu$W)}\end{tabular} &
  \textbf{GE} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Throughput}\\  \textbf{(@ 100 KHz)}\\ \textbf{(Kbps)}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Figure of Merit}\\  \textbf{(FoM)} \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{CMOS} \\ \textbf{Tech}\\ \textbf{($\mu$m)}\end{tabular} \\ \midrule
  
\multirow{6}{*}{\rotatebox{90}{\makecell{Merkle Dåmgard \\ Construction}}} & PRESENT~\cite{aumasson2013quark}  & DM-PRESENT-80  & 2008 & 64  & 1.83 & 1600 & 14.63 & 57.15 & 0.18 \\
            &  & DM-PRESENT-128 &      & 64  & 2.94 & 1886 & 22.9  & 64.38 &      \\
            &  & H-PRESENT-128  &      & 128 & 6.44 & 2330 & 11.45 & 21.09 &     \\
            &  & C-PRESENT-192  &      & 192 &      & 4600 & 1.9   & 0.9   &     \\ \cline{2-10} \\

& Lesamnta-LW~\cite{el2022survey} &                & 2010 & 256 &      & 8240 &       &       &0.09 \\  \hline

\multirow{21}{*}{\rotatebox{90}{\makecell{Sponge \\ Construction}}} & QUARK~\cite{aumasson2013quark}     & U-QUARK        & 2010 & 128 & 2.44 & 1379 & 1.47  & 7.73  & 0.18 \\
            &  & D-QUARK        &      & 160 & 3.10 & 1702 & 2.27  & 7.84  &     \\
            &  &S-QUARK        &      & 224 & 4.35 & 2296 & 3.13  & 5.94  &     \\ \cline{2-10}
            

& PHOTON~\cite{guo2011photon}      & PHOTON-80      & 2011 & 80  & 1.59 & 865  & 2.82  &  37.69 & 0.18 \\
            &  & PHOTON-128     &      & 128 & 2.29 & 1122 & 1.61  &  12.79 &    \\
            &  & PHOTON-160     &      & 160 & 2.74 & 1396 & 2.70  &  13.85 &    \\
            &  & PHOTON-224     &      & 224 & 4.01 & 1736 & 1.86  &  6.17  &    \\
            &  & PHOTON-256     &      & 256 & 4.55 & 2177 & 3.21  &  6.77  &  \\ \cline{2-10}
            
& SPONGENT~\cite{bogdanov2011spongent}    & SPONGENT-88    & 2011 & 88  & 1.57 & 738  & 0.81  &  14.87  & 0.13 \\
            &  & SPONGENT-128   &      & 128 & 2.20 & 1060 & 0.34  &  3.03   &      \\
            &  & SPONGENT-160   &      & 160 & 2.85 & 1329 & 0.40  &  2.26   &    \\
            &  & SPONGENT-224   &      & 224 & 3.73 & 1728 & 0.22  &  0.74   &    \\
            &  & SPONGENT-256   &      & 256 & 6.62 & 1950 & 0.17  &  0.45   &    \\ \cline{2-10}
            
& GLUON~\cite{berger2012gluon}       & GLUON-64       & 2012 & 128 &      & 2071 & 12.12 &  28.26  & 0.13 \\
            &  & GLUON-80       &      & 160 &      & 2799 & 32    &  40.85  &    \\
            &  & GLUON-112      &      & 224 &      & 4724 & 58.18 &  26.07  &    \\ \cline{2-10}
            
& LHash~\cite{wu2013lhash}       & LHash-80       & 2013 & 96  &      & 817  & 2.40  & 35.96   & 0.18 \\
            &  & LHash-96       &      & 128 &      & 817  & 2.40  & 35.96   &     \\
            &  & LHash-128      &      & 160 &      & 1028 & 1.81  & 17.13   &  \\ \cline{2-10}

& Neeva-Hash~\cite{bussi2016neeva}  &                & 2016 & 224 &      &      & 4.99  &      \\ \cline{2-10}

& Hash-One~\cite{megha2016hash}    &                & 2016 & 160 &      & 1006 &       &       & 0.18 \\ \hline

& BLAKE2~\cite{sklavos2010blake}      & BLAKE2b        & 2013 & 512 &      &      &       &      \\
            &  & BLAKE2s        &      & 256 &      &      &       &      \\ \hline

& LNHASH~\cite{9066107}     & LNHASH-96      & 2019 & 96  &      & 927  &       &       & 0.18 \\
            &  & LNHASH-128     &      & 128 &      & 1224 &       &      \\
            &  & LNHASH-160     &      & 160 &      & 1539 &       &      \\  \bottomrule
\end{tabular*}
\label{tab:HW_imp_LWHF}
\end{table}

==> Tables/03.Software_Implementation_Tables/09_SW_Metrics_LWHF.tex <==
\begin{table} [H]
\scriptsize
\caption{Software Implementation of Lightweight Hash Functions (LWHF).}
\label{tab:SW_imp_LWHF}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}} l l c c c c c  }
\toprule
\multicolumn{2}{l}{\textbf{Hash Function}} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Collision} \\ \textbf{Resistance}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Hash}\\  \textbf{Size}\\ \textbf{(bits)}\end{tabular} &
  \begin{tabular}[c]{@{}c@{}} \textbf{Cycles/byte} \\ \textbf{(CpB)} \end{tabular} &
  \begin{tabular}[c]{@{}c@{}} \textbf{Power Consumption} \\ ($\mu$W) \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\textbf{Hardware} \\ \textbf{Config} \end{tabular} 
                      
\\ 
\midrule

Lesamnta-LW  &             & $2^{128}$    & 256 & 146925   &       &  
\multirow{18}{*}{\rotatebox{90}{\makecell{ Intel Core 3 \\(64-bit)\\~\cite{nabeel2021security}}}}      \\ \cline{1-6}

QUARK         & U-QUARK    & $2^{64}$    & 128 & 151992    & 8.44  &  \\              
              & D-QUARK    & $2^{80}$     & 160 & 170231   & 8.90  &      \\
              & T-QUARK    & $2^{112}$    & 224 & 173705   & 8.95  &      \\ \cline{1-6}   

PHOTON        & PHOTON-80  & $2^{40}$   & 80  & 51880    & 6.59  &      \\
              & PHOTON-128 & $2^{64}$   & 128 & 121593   & 7.29  &      \\
              & PHOTON-160 & $2^{80}$   & 160 & 137806   & 7.99  &      \\
              & PHOTON-224 & $2^{112}$  & 224 & 138964   & 8.01  &      \\
              & PHOTON-256 & $2^{128}$  & 256 & 162125   & 8.8   &      \\ \cline{1-6}

SPONGENT      & SPONGENT-88  & $2^{40}$   & 88  & 66324    & 5.87  &      \\
              & SPONGENT-128 & $2^{64}$   & 128 & 121992   & 7.28  &      \\
              & SPONGENT-160 & $2^{80}$   & 160 & 159700   & 8.82  &      \\
              & SPONGENT-224 & $2^{112}$  & 224 & 153439   & 8.94  &      \\
              & SPONGENT-256 & $2^{128}$  & 256 & 177324   & 9.4   &      \\ \cline{1-6}

LNMNT        & LNMNT-80  & $2^{50}$     & 80  & 51180    & 5.52  &      \\
              & LNMNT-128 & $2^{80}$    & 128 & 52042    & 6.57  &      \\
              & LNMNT-160 & $2^{100}$   & 160 & 52742    & 6.68  &      \\
              & LNMNT-224 & $2^{140}$   & 224 & 55260    & 6.82  &      \\ \hline

QUARK         & U-QUARK    & $2^{64}$    & 128  & 43373     &      & \multirow{7}{*}{\rotatebox{90}{\makecell{ Intel Core 2 Duo \\(64-bit)\\~\cite{berger2012gluon, bussi2016neeva}}}}     \\              
              & D-QUARK    & $2^{80}$     & 160 & 35103     &      &      \\
              & T-QUARK    & $2^{112}$    & 224 & 25142     &      &      \\ \cline{1-6}

GLUON        & GLUON-64  & $2^{64}$    & 128  & 17319      &       &      \\
              & GLUON-80 & $2^{80}$    & 160  & 8523       &       &      \\
              & GLUON-112 & $2^{112}$   & 224 & 1951       &       &      \\ \cline{1-6}

Neeva-Hash   &           & $2^{112}$    & 224  & 12067     &       &      \\ \hline

PHOTON        & PHOTON-80  & $2^{40}$   & 80  & 96    &     & \multirow{5}{*}{\makecell{Intel i7-3612QM \\ (64-bit)\\~\cite{wu2014lhash}}}     \\
              & PHOTON-128 & $2^{64}$   & 128 & 156   &     &      \\ \cline{1-6}

LHash        & LHash-80  & $2^{48}$     & 96  & 139    &     &      \\
              & LHash-96 & $2^{64}$     & 128 & 139    &     &      \\
              & LHash-128 & $2^{80}$   & 160 & 156    &     &      \\

\bottomrule
\end{tabular*}
\end{table}
